Is AI Art Another Industrial Revolution in the Making?

A major shift from skilled to unskilled workers was one of the many changes caused by the Industrial Revolution, when the switch to machines contributed to decline in the social and economic status of artisans, whose skills were dismembered into discrete actions by factory-line workers. We consider what may be an analogous computing technology: the recent introduction of AI-generated art software. AI art generators such as Dall-E and Midjourney can create fully rendered images based solely on a user's prompt, just at the click of a button. Some artists fear if the cheaper price and conveyor-belt speed that comes with AI-produced images is seen as an improvement to the current system, it may permanently change the way society values/views art and artists. In this article, we consider the implications that AI art generation introduces through a post-industrial revolution historical lens. We then reflect on the analogous issues that appear to arise as a result of the AI art revolution, and we conclude that the problems raised mirror those of industrialization, giving a vital glimpse into what may lie ahead.

==> todo_and_delete.tex <==
Before we upload and once everything is done,


- To add politcal (kd/al)
- To add plagiarism (kd)
- conclusion/coherence


- Verify for hype (avoid words like fear..)..kd

- Note that quotes start with `` and end with ''..kd

- Verify that words like AI and AI art are not used loosely ..kd

- Most Important: Is our paper able to convey a takeaway message (need not necessarily be recommendations) ? Verify/Edit for Coherence..alexis

- Most Important: Verify if Title, Abstract, Introduction & Conclusion are aligned..alexis/kd

- Most Important: Verify for citations (of dall-e, stable diffusion, etc)..alexis..

---------------- Reviews ------------
concern of reviewer 2:
- the industrial revolution for a period in which artisans found themselves out of work en masse thanks to the introduction of dedicated equipment for the production of goods. Perhaps inspired by the surface-level similarity between the words “artist” and “artisan,” the authors ask whether AI will similarly push artists out of work. Their analysis is unsatisfying. --> 
(KD: limitations)
TODO: mention in the conclusion or limitations section about that a more thorough analysis with empirical evidence can strengthen some of the arguments. Our paper is intended to spur up discussions....


1) The authors fail to disambiguate what sort of 'art' they are engaging with. Their haphazard invocation of the term indicates a confusion over the difference between fine art (institutionalized art, contemporary art, etc.) and commercial art (illustrations, graphics, kitsch, etc.). 
(KD: limitations)
TODO: mention these words explicitly in at least fast-paced computational creativity, reduced dependency on, benefits to business...


2) We recommend the authors read Walter Benjamin, Theodor Adorno, and Max Horkheimer for an introduction to the study of mass-produced art. What technological innovations mean for art has been discussed extensively. (KD & AN)

3) Artists are not artisans, and neither is the industrial revolution equivalent to the “AI revolution.” Artists do art, artisans do crafts. Artisans were employed prior to the industrial revolution because society was primarily agrarian—artisans and their corresponding guilds were responsible for the production of nearly all goods, unlike artists; who are preoccupied with art. “AI-based art models” are not arriving in an empty environment. Freelance artists have been working in a digital environment where tools partially responsible for the artwork have been around for a long while (Blender, Photoshop, and so on). This is not mentioned.
(Alexis)
TODO: this is something to mention about...


4) The authors persistently undermine their own analysis. An example is found in their comparison between contemporary artists and industrial revolution-era artisans, where the authors point out artisans both survived and, indeed, thrived following industrialization (“the global market for artisan-made products has increased…”). This fact is not recalled in the conclusion, where the authors suggest the artist will be deprecated just as the “artisan was pushed out.”
TODO: this definitely needs to be addressed.

5) typo in the title -> “Effects of AI Art : Another…”
'an artist is not made just by putting pen to paper’—should be 'art'?
general punctuation errors throughout
disambiguate what is meant by ‘art’ and ‘artist’
(KD)

6) language is unacademic, e.g. “It is crystal clear,” “unarguably” 
(KD)
TODO: crystal clear can be changed. unarguably is fine.


7) Title TODO: change
Is AI Art Another Industrial Revolution in the Making?

8) Acknolwledgments : Kristin W, Steve Newton, 


titles
%\title{Effects of AI Art : Another Industrial Revolution in the Making}
\title{Is AI Art Another Industrial Revolution in the Making?}
%\title{Does AI Art Indicate Another Industrial Revolution in the Making?}
% AI Art - Unfolding of the Industrial Revolution 
% 
